HUMANO: A Large-Scale Benchmark for Generalist Humanoid Loco-Manipulation

Recent advances in vision-language-action models and whole-body control have rapidly expanded the capabilities of humanoid loco-manipulation, enabling generalist policies to perform increasingly diverse tasks with a single model. However, existing benchmarks often focus on individual tasks or small task suites, making it difficult to systematically evaluate multi-task capabilities and generalization. To fill this gap, we present HUMANO, a large-scale benchmark for generalist humanoid loco-manipulation. HUMANO contains 100 tasks organized into eight complementary suites, spanning 90 interactive scenes and over 2K object assets, with 5K in-distribution whole-body demonstrations. The benchmark covers fundamental skills, goal-directed loco-manipulation, generalization across spatial configurations, objects, robot configurations, and goals, as well as long-horizon skill composition and state-dependent reasoning. HUMANO further provides 30K OOD demonstrations covering six non-linguistic distribution shifts (distractors, lighting, background, camera viewpoint, sensor noise, and robot initialization), along with 17.5K evaluation episodes across all seven OOD settings, including language variation. All policies operate through a shared SONIC-based motion-latent interface, enabling standardized comparison under a common whole-body execution framework. Experiments with representative imitation and vision-language-action policies demonstrate the emerging potential of generalist models for multi-task humanoid loco-manipulation. Although multi-task learning remains more challenging than single-task training, performance continues to improve with increasing demonstration scale. Preliminary sim-to-real results show that policies trained on HUMANO simulation data can transfer executable whole-body behaviors to a physical humanoid robot.

==> sections/4-model.tex <==
\section{Model Design}
\label{sec:model}

% 暂未设计


==> sections/7-AI_use_statement.tex <==
\subsection*{AI use statement}

In this work, we used generative AI tools for language editing, including grammar correction, sentence refinement, and improving the clarity and readability of the manuscript. We have not used generative AI tools for generating research ideas, designing experiments, collecting or analyzing data, deriving scientific claims, or producing experimental results.
Additionally, we used generative AI tools for recommended disclosure tasks related to writing assistance. All AI-assisted edits were carefully reviewed and revised by the authors. The authors verified the accuracy, consistency, and originality of the final manuscript, and take full responsibility for all content, including text, claims, and artifacts presented in this work.

==> sections/acknowledgments.tex <==
\subsubsection*{Acknowledgments}

==> tables/ablation_post-train_data.tex <==
\begin{table*}[t]
\centering
\small
\caption{
Multi-task scaling results of GR00T N1.7 on the Movement suite.
We report success rate (\%) when training with 5, 10, 25, and 50 demonstrations per task.
\textbf{Bold} denotes the best result for each task.
}
\label{tab:post-train_scaling}
\vskip -0.05in
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccc}
\toprule
\makecell{Demos\\per Task} &
Avg. &
\makecell{Ball\\Kick} &
\makecell{Chair\\Push} &
\makecell{Chair\\Sit} &
\makecell{Dolly\\Push} &
\makecell{Ground\\Basket Pick} &
\makecell{Ground\\Bottle Pick} &
\makecell{Ground\\Box Pick} &
\makecell{Table\\Apple Pick} &
\makecell{Table\\Book Pick} &
\makecell{Table\\Plate Pick} \\
\midrule
5
& 0.0
& 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\

10
& 29.6
& 20 & 96 & 0 & \textbf{64} & 52 & 0 & \textbf{52} & 0 & 12 & 0 \\

25
& 30.0
& 20 & 96 & 24 & 44 & 32 & \textbf{4} & 40 & 0 & 16 & 24 \\

50
& \textbf{39.2}
& \textbf{24} & \textbf{100} & \textbf{56} & 8 & \textbf{76}
& \textbf{4} & 20 & \textbf{12} & \textbf{48} & \textbf{44} \\
\bottomrule
\end{tabular}
}
\end{table*}
